Enhancing Stability in Training Conditional Generative Adversarial Networks via Selective Data Matching

Conditional generative adversarial networks (cGANs) have demonstrated remarkable success due to their class-wise controllability and superior quality for complex generation tasks. Typical cGANs solve the joint distribution matching problem by decomposing two easier sub-problems: marginal matching and conditional matching. In this paper, we proposes a simple but effective training methodology, selective focusing learning, which enforces the discriminator and generator to learn easy samples of each class rapidly while maintaining diversity. Our key idea is to selectively apply conditional and joint matching for the data in each mini-batch.Specifically, we first select the samples with the highest scores when sorted using the conditional term of the discriminator outputs (real and generated samples). Then we optimize the model using the selected samples with only conditional matching and the other samples with joint matching. From our toy experiments, we found that it is the best to apply only conditional matching to certain samples due to the content-aware optimization of the discriminator. We conducted experiments on ImageNet (64x64 and 128x128), CIFAR-10, CIFAR-100 datasets, and Mixture of Gaussian, noisy label settings to demonstrate that the proposed method can substantially (up to 35.18% in terms of FID) improve all indicators with 10 independent trials. Code is available at https://github.com/pnu-cvsp/Enhancing-Stability-in-Training-Conditional-GAN-via-Selective-Data-Matching.

==> 2_preliminary.tex <==
\subsection{Conditional Generative Adversarial Networks}
% \textcolor{Orchid}{
% A generative adversarial network (GAN) (Goodfellow et al., 2014) consists of two separate neural networks — a generator, and a discriminator. The generator G takes as input a sample from the prior z ∈ Z ∼ $p_z$ and produces a sample G(z) ∈ X. The discriminator takes an observation x ∈ X as input and produces a probability D(x) that the observation is real. The observation is sampled either according to the density $p_{data}$ (the data generating distribution) or $p_g$ (the implicit density given by the generator and the prior).}
% \textbf{Conditional GANs}
% Projection discriminator 논문과 Mining GOLD 논문 섞어서 작성 (경훈)
% GAN loss부터 cGAN 설명하고 GOLD 논문보고 Marginal term과 conditional term으로 나누는 내용까지 넣기
% skyblue =>DISCRIMINATOR REJECTION SAMPLING 
% Emerald =>Mining GOLD
% brown => big gan
% \textcolor{brown}{In conditional GANs (Mirza & Osindero, 2014) class information can be fed into the model in various ways.}
The goal of cGANs is to learn the model distribution $p_g(x, y)$ to match with the real data distribution $p_{data}(x, y)$. To this end, various architectures have been proposed to incorporate additional attributes \citep{mirza2014conditional,odena2017ACGAN,miyato2018project}. The generator G : (z, y) → x maps a pair of a latent z and an attribute y to generate a sample x whereas the discriminator D guides the generator to learn the joint distribution p(x, y). The standard adversarial loss for the discriminator is given by
\begin{multline}
% \begin{split}
 \mathcal{L}_{D} =\,-\; \mathbb{E}_{(x,y)\sim p_{data}(x,y)}[\log{D(x,y)}]\\
   -\,\mathbb{E}_{(z,y)\sim p_{g}(z,y)}[\log(1-D(G(z,y)))].\quad\;\;
  \label{eq:ganloss}
%   \end{split}
\end{multline}
By observing the form of the optimal solution \citep{goodfellow2014generative} for the loss function, \eqref{eq:ganloss} can be decomposed into a sum of two log likelihood ratios as follows.
\begin{multline}
% \begin{split}
 {f(x,y)} = {\log{\frac{p_{data}(x|y)p_{data}(y)}{p_g(x|y)p_g(y)}}} \\ = {\underbrace{\log{\frac{p_{data}(y|x)}{p_g(y|x)}}}_{conditional}+  \underbrace{\log{\frac{p_{data}(x)}{p_g(x)}}}_{marginal}}.\qquad\quad\;\;
  \label{eq:cganloss}
%   \end{split}
\end{multline}


%\begin{align*}
% \log{p_{data}(x,y)}-\log{p_g(x,y)} &= {\log{\frac{p_{data}(x,y)}{p_g(x,y)}}} \\
% &= {\log{\frac{p_{data}(x|y)p_{data}(y)}{p_g(x|y)p_g(y)}}} \\&= {\underbrace{\log{\frac{p_{data}(y|x)}{p_g(y|x)}}}_{conditional}+  \underbrace{\log{\frac{p_{data}(x)}{p_g(x)}}}_{marginal}}.
%  \label{eq:cganloss}
%\end{align*}

% In this paper, we will look closely into the conditional term by empirical (Section \ref{Observations}) and theoretical (Section \ref{Theoretical Perspectives}).
In this paper, we will look closely into the conditional term with empirical (Section \ref{Observations}) and theoretical (Section \ref{Theoretical Perspectives}).
% := \underbrace{r(y|x)}_{conditional}+\underbrace{r(x)}_{marginal}
% projection discriminator 정확하게 유도한 내용은 Quick analysis에 넣을 예정
% \textbf{Instance Selection for GANs}
% 여기는 embedding하고 scoring 간단하게 설명
% Collaboration에서 이 score 사용하기 때문에 설명 필요. 여기 넣을지 뒤에 넣을지는 고민해보자

% More precisely, given a dataset of images $S$ , the data set of embedded images Z is obtained by applying the embedding function z = F(x) to each data point x ∈ $S$. For the task of image generation we suggest using perceptually aligned embedding functions \citep{zhang2018unreasonable}, such as the feature space of a pretrained image classifier. 



==> check_list.tex <==
%%% BEGIN INSTRUCTIONS %%%
\newpage
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{Conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{Broader Impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section Appendix B.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{We have dealt with the analysis and interpretation of the phenomenon.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See the algorithm \ref{alg:example} and we submit the code URL in Appendix E.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See in Appendix C.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Table \ref{Performance_SAGAN}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section \ref{Experiments on ImageNet}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Cite all assets we use.}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We followed the guidelines of people whose data.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We used datasets without personally identifiable information.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
